Saying Hello World with GROOVE - A Solution to the TTC 2011 Instructive Case

This report presents a solution to the Hello World case study of TTC 2011 using GROOVE. We provide and explain the grammar that we used to solve the case study. Every requested question of the case study was solved by a single rule application.

==> eptcsdata.tex <==
\providecommand{\firstpage}{215}
\providecommand{\publicationstatus}{Van Gorp, Mazanek and Rose (Eds.): \\Fifth Transformation Tool Contest (TTC 2011)\\
EPTCS 74, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.74.19}{10.4204/EPTCS.74.19}}
\pdfoutput=1

